A Comparative Study of Programming Languages in Rosetta Code

Sometimes debates on programming languages are more religious than scientific. Questions about which language is more succinct or efficient, or makes developers more productive are discussed with fervor, and their answers are too often based on anecdotes and unsubstantiated beliefs. In this study, we use the largely untapped research potential of Rosetta Code, a code repository of solutions to common programming tasks in various languages, to draw a fair and well-founded comparison. Rosetta Code offers a large data set for analysis. Our study is based on 7087 solution programs corresponding to 745 tasks in 8 widely used languages representing the major programming paradigms (procedural: C and Go; object-oriented: C# and Java; functional: F# and Haskell; scripting: Python and Ruby). Our statistical analysis reveals, most notably, that: functional and scripting languages are more concise than procedural and object-oriented languages; C is hard to beat when it comes to raw speed on large inputs, but performance differences over inputs of moderate size are less pronounced and allow even interpreted languages to be competitive; compiled strongly-typed languages, where more defects can be caught at compile time, are less prone to runtime failures than interpreted or weakly-typed languages. We discuss implications of these results for developers, language designers, and educators.

==> binsize_exit0_mean_network.tex <==
\node [lang] (C) at (-3.94756232346801,0) {C};
\node [lang] (C-sharp) at (8.68537394080806,0) {C\#};
\node [lang] (F-Sharp) at (2.36706373572394,0) {F\#};
\node [lang] (Go) at (-15,0) {Go};
\node [lang] (Haskell) at (-9.20852265749723,0) {Haskell};
\node [lang] (Java) at (11.3158541078227,0) {Java};
\node [lang] (Python) at (15,0) {Python};
\draw [->,,colorstrong](C) edge (F-Sharp);
\draw [->,,colorstrong](Haskell) edge (C);
\draw [->,,colorstrong](F-Sharp) edge (C-sharp);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colorstrong](Go) edge (Haskell);
\draw [->,,colorweak](Java) edge (Python);


==> binsize_exit0_mean_normrank_network.tex <==
\node [lang] (C) at (14.8736434307412,0) {C};
\node [lang] (C-sharp) at (14.9786412499679,6) {C\#};
\node [lang] (F-Sharp) at (14.9320753264746,3) {F\#};
\node [lang] (Go) at (-15,0) {Go};
\node [lang] (Haskell) at (-5.85351617620648,0) {Haskell};
\node [lang] (Java) at (14.9876850450266,9) {Java};
\node [lang] (Python) at (15,12) {Python};
\draw [->,,colorstrong](C) edge (F-Sharp);
\draw [->,,colorstrong](Haskell) edge (C);
\draw [->,,colorstrong](F-Sharp) edge (C-sharp);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colorstrong](Go) edge (Haskell);
\draw [->,,colorweak](Java) edge (Python);


==> binsize_exit0_min_network.tex <==
\node [lang] (C) at (-5.17016654598117,0) {C};
\node [lang] (C-sharp) at (8.27661115133961,0) {C\#};
\node [lang] (F-Sharp) at (2.07096307023896,0) {F\#};
\node [lang] (Go) at (-15,0) {Go};
\node [lang] (Haskell) at (-9.30847212165098,0) {Haskell};
\node [lang] (Java) at (11.3794351918899,0) {Java};
\node [lang] (Python) at (15,0) {Python};
\draw [->,,colorstrong](C) edge (F-Sharp);
\draw [->,,colorstrong](Haskell) edge (C);
\draw [->,,colorstrong](F-Sharp) edge (C-sharp);
\draw [->,,colorweak](C-sharp) edge (Java);
\draw [->,,colorstrong](Go) edge (Haskell);
\draw [->,,colorweak](Java) edge (Python);


==> binsize_exit0_min_normrank_network.tex <==
\node [lang] (C) at (14.8742502174612,0) {C};
\node [lang] (C-sharp) at (14.9798619040321,6) {C\#};
\node [lang] (F-Sharp) at (14.9333046982415,3) {F\#};
\node [lang] (Go) at (-15,0) {Go};
\node [lang] (Haskell) at (-5.66434132453848,0) {Haskell};
\node [lang] (Java) at (14.989898575656,9) {Java};
\node [lang] (Python) at (15,12) {Python};
\draw [->,,colorstrong](C) edge (F-Sharp);
\draw [->,,colorstrong](Haskell) edge (C);
\draw [->,,colorstrong](F-Sharp) edge (C-sharp);
\draw [->,,colorweak](C-sharp) edge (Java);
\draw [->,,colorstrong](Go) edge (Haskell);
\draw [->,,colorweak](Java) edge (Python);


==> commentstocode_any_mean_normrank_network.tex <==
\node [lang] (C) at (-11.6447368421053,0) {C};
\node [lang] (C-sharp) at (-15,0) {C\#};
\node [lang] (F-Sharp) at (15,0) {F\#};
\node [lang] (Go) at (-11.8421052631579,3) {Go};
\node [lang] (Haskell) at (-8.48684210526316,0) {Haskell};
\node [lang] (Java) at (-14.4078947368421,3) {Java};
\node [lang] (Python) at (-9.47368421052632,6) {Python};
\node [lang] (Ruby) at (-4.3421052631579,0) {Ruby};
\draw [->,,colormedium](C) edge (Go);
\draw [->,dotted,thick,colormedium,bend right=20](C) edge (Ruby);
\draw [->,,colormedium](C-sharp) edge (Go);
\draw [->,dotted,thick,colormedium,bend right=20](C-sharp) edge (Haskell);
\draw [->,,colormedium](C-sharp) edge (Python);
\draw [->,dotted,thick,colormedium,bend right=20](Haskell) edge (F-Sharp);
\draw [->,,colormedium](Python) edge (F-Sharp);
\draw [->,dotted,thick,colormedium](Ruby) edge (F-Sharp);
\draw [->,,colormedium](Java) edge (Go);
\draw [->,,colormedium](Java) edge (Haskell);
\draw [->,,colormedium](Java) edge (Python);


==> commentstocode_any_min_normrank_network.tex <==
\node [lang] (C) at (-13,0) {C};
\node [lang] (C-sharp) at (-13.6,3) {C\#};
\node [lang] (F-Sharp) at (15,0) {F\#};
\node [lang] (Go) at (-11.6,0) {Go};
\node [lang] (Haskell) at (-8.2,0) {Haskell};
\node [lang] (Java) at (-15,6) {Java};
\node [lang] (Python) at (-11.8,3) {Python};
\node [lang] (Ruby) at (-7.6,3) {Ruby};
\draw [->,dotted,thick,colormedium](C-sharp) edge (C);
\draw [->,,colormedium](C) edge (Go);
\draw [->,dotted,thick,colormedium](C) edge (Ruby);
\draw [->,dotted,thick,colormedium,bend right=20](Go) edge (F-Sharp);
\draw [->,,colormedium](Haskell) edge (F-Sharp);
\draw [->,,colormedium](Python) edge (F-Sharp);
\draw [->,,colormedium](Ruby) edge (F-Sharp);
\draw [->,,colormedium](Java) edge (Go);
\draw [->,,colormedium](Java) edge (Haskell);
\draw [->,,colormedium](Java) edge (Ruby);


==> corr_stats_stat_network.tex <==
\node [lang] (C) at (-0.517241379310343,0) {C};
\node [lang] (C-sharp) at (-13.9655172413793,0) {C\#};
\node [lang] (F-Sharp) at (13.9655172413793,0) {F\#};
\node [lang] (Go) at (15,0) {Go};
\node [lang] (Haskell) at (-15,3) {Haskell};
\node [lang] (Java) at (-0.517241379310343,3) {Java};
\node [lang] (Python) at (-1.55172413793103,6) {Python};
\node [lang] (Ruby) at (6.72413793103448,0) {Ruby};
\draw [->,,colorweak](C-sharp) edge (C);
\draw [->,,colorweak](Haskell) edge (C);
\draw [->,dotted,thick,colormedium](C) edge (Ruby);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colorweak](C-sharp) edge (Python);
\draw [->,dotted,thick,colormedium](Ruby) edge (F-Sharp);
\draw [->,,colormedium,bend right=20](Ruby) edge (Go);
\draw [->,,colorweak](Haskell) edge (Java);
\draw [->,,colorweak](Haskell) edge (Python);
\draw [->,dotted,thick,colormedium](Java) edge (Ruby);
\draw [->,,colormedium](Python) edge (Ruby);


==> loc_any_mean_network.tex <==
\node [lang] (C) at (-15,0) {C};
\node [lang] (C-sharp) at (-15,3) {C\#};
\node [lang] (F-Sharp) at (12.6,0) {F\#};
\node [lang] (Go) at (-13.8,6) {Go};
\node [lang] (Haskell) at (15,3) {Haskell};
\node [lang] (Java) at (-6.6,0) {Java};
\node [lang] (Python) at (13.8,6) {Python};
\node [lang] (Ruby) at (13.8,9) {Ruby};
\draw [->,,colormedium](C) edge (Java);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colorweak](Java) edge (F-Sharp);
\draw [->,,colormedium](Go) edge (Java);
\draw [->,,colorstrong](Java) edge (Haskell);
\draw [->,,colorweak](Java) edge (Python);
\draw [->,,colorstrong](Java) edge (Ruby);


==> loc_any_mean_normrank_network.tex <==
\node [lang] (C) at (-15,0) {C};
\node [lang] (C-sharp) at (-8.03571428571429,0) {C\#};
\node [lang] (F-Sharp) at (14.1766538830297,0) {F\#};
\node [lang] (Go) at (-10.2289069990412,0) {Go};
\node [lang] (Haskell) at (14.496644295302,3) {Haskell};
\node [lang] (Java) at (-2.40172579098754,0) {Java};
\node [lang] (Python) at (15,6) {Python};
\node [lang] (Ruby) at (13.4252157238734,9) {Ruby};
\draw [->,,colormedium,bend right=20](C) edge (Java);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colorweak](Java) edge (F-Sharp);
\draw [->,,colormedium,bend right=20](Go) edge (Java);
\draw [->,,colorstrong](Java) edge (Haskell);
\draw [->,,colorweak](Java) edge (Python);
\draw [->,,colorstrong](Java) edge (Ruby);


==> loc_any_min_network.tex <==
\node [lang] (C) at (-13.8461538461538,0) {C};
\node [lang] (C-sharp) at (-15,3) {C\#};
\node [lang] (F-Sharp) at (10.3846153846154,0) {F\#};
\node [lang] (Go) at (-13.8461538461538,6) {Go};
\node [lang] (Haskell) at (13.8461538461538,0) {Haskell};
\node [lang] (Java) at (-9.23076923076923,0) {Java};
\node [lang] (Python) at (15,3) {Python};
\node [lang] (Ruby) at (12.6923076923077,6) {Ruby};
\draw [->,,colormedium](C) edge (Java);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colorweak](Java) edge (F-Sharp);
\draw [->,,colormedium](F-Sharp) edge (Python);
\draw [->,,colormedium](Go) edge (Java);
\draw [->,,colorstrong,bend right=20](Java) edge (Haskell);
\draw [->,,colorstrong](Java) edge (Ruby);


==> loc_any_min_normrank_network.tex <==
\node [lang] (C) at (-15,0) {C};
\node [lang] (C-sharp) at (-11.8324788693363,0) {C\#};
\node [lang] (F-Sharp) at (11.0218927532216,0) {F\#};
\node [lang] (Go) at (-14.8378827767771,3) {Go};
\node [lang] (Haskell) at (12.8342801718165,0) {Haskell};
\node [lang] (Java) at (-3.92198974643204,0) {Java};
\node [lang] (Python) at (15,3) {Python};
\node [lang] (Ruby) at (12.9963973950395,6) {Ruby};
\draw [->,,colormedium,bend right=20](C) edge (Java);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colorweak](Java) edge (F-Sharp);
\draw [->,,colormedium](F-Sharp) edge (Python);
\draw [->,,colormedium](Go) edge (Java);
\draw [->,,colorstrong,bend right=20](Java) edge (Haskell);
\draw [->,,colorstrong](Java) edge (Ruby);


==> loc_exit0_mean_network.tex <==
\node [lang] (C) at (-11.7857142857143,0) {C};
\node [lang] (C-sharp) at (-15,0) {C\#};
\node [lang] (F-Sharp) at (11.7857142857143,0) {F\#};
\node [lang] (Go) at (-15,3) {Go};
\node [lang] (Haskell) at (15,0) {Haskell};
\node [lang] (Java) at (-8.57142857142857,0) {Java};
\node [lang] (Python) at (11.7857142857143,3) {Python};
\node [lang] (Ruby) at (11.7857142857143,6) {Ruby};
\draw [->,,colormedium](Java) edge (C);
\draw [->,,colormedium,bend right=20](C-sharp) edge (Java);
\draw [->,,colorweak](Java) edge (F-Sharp);
\draw [->,dotted,thick,colormedium](Go) edge (Java);
\draw [->,,colorstrong,bend right=20](Java) edge (Haskell);
\draw [->,,colorweak](Java) edge (Python);
\draw [->,,colorweak](Java) edge (Ruby);


==> loc_exit0_mean_normrank_network.tex <==
\node [lang] (C) at (-15,0) {C};
\node [lang] (C-sharp) at (-14.3300601837187,3) {C\#};
\node [lang] (F-Sharp) at (14.6579030725372,0) {F\#};
\node [lang] (Go) at (-11.9021222679759,0) {Go};
\node [lang] (Haskell) at (14.7101678808996,3) {Haskell};
\node [lang] (Java) at (-10.7142857142857,3) {Java};
\node [lang] (Python) at (15,6) {Python};
\node [lang] (Ruby) at (12.1824516946468,9) {Ruby};
\draw [->,,colormedium](Java) edge (C);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colorweak](Java) edge (F-Sharp);
\draw [->,dotted,thick,colormedium](Go) edge (Java);
\draw [->,,colorstrong](Java) edge (Haskell);
\draw [->,,colorweak](Java) edge (Python);
\draw [->,,colorweak](Java) edge (Ruby);


==> loc_exit0_min_network.tex <==
\node [lang] (C) at (-13,0) {C};
\node [lang] (C-sharp) at (-15,3) {C\#};
\node [lang] (F-Sharp) at (9,0) {F\#};
\node [lang] (Go) at (-14,6) {Go};
\node [lang] (Haskell) at (13,0) {Haskell};
\node [lang] (Java) at (-7,0) {Java};
\node [lang] (Python) at (15,3) {Python};
\node [lang] (Ruby) at (12,9) {Ruby};
\draw [->,dotted,thick,colormedium](C) edge (Java);
\draw [->,,colorweak](C-sharp) edge (Java);
\draw [->,,colorstrong](Java) edge (F-Sharp);
\draw [->,,colorweak](F-Sharp) edge (Python);
\draw [->,dotted,thick,colormedium](F-Sharp) edge (Ruby);
\draw [->,dotted,thick,colormedium](Go) edge (Java);
\draw [->,,colorstrong,bend right=20](Java) edge (Haskell);
\draw [->,dotted,thick,colormedium](Haskell) edge (Python);


==> loc_exit0_min_normrank_network.tex <==
\node [lang] (C) at (-14.5348465473146,0) {C};
\node [lang] (C-sharp) at (-15,3) {C\#};
\node [lang] (F-Sharp) at (12.2858056265985,0) {F\#};
\node [lang] (Go) at (-13.1969309462916,6) {Go};
\node [lang] (Haskell) at (13.4846547314578,3) {Haskell};
\node [lang] (Java) at (-9.81617647058823,0) {Java};
\node [lang] (Python) at (15,6) {Python};
\node [lang] (Ruby) at (13.2544757033248,9) {Ruby};
\draw [->,dotted,thick,colormedium](C) edge (Java);
\draw [->,,colorweak](C-sharp) edge (Java);
\draw [->,,colorstrong](Java) edge (F-Sharp);
\draw [->,,colorweak](F-Sharp) edge (Python);
\draw [->,dotted,thick,colormedium](F-Sharp) edge (Ruby);
\draw [->,dotted,thick,colormedium](Go) edge (Java);
\draw [->,,colorstrong](Java) edge (Haskell);
\draw [->,dotted,thick,colormedium](Haskell) edge (Python);


==> make_stats_stat_network.tex <==
\node [lang] (C) at (-1.45161290322581,0) {C};
\node [lang] (C-sharp) at (-6.29032258064516,0) {C\#};
\node [lang] (F-Sharp) at (11.1290322580645,0) {F\#};
\node [lang] (Go) at (6.29032258064516,0) {Go};
\node [lang] (Haskell) at (-15,0) {Haskell};
\node [lang] (Java) at (-4.35483870967742,0) {Java};
\node [lang] (Python) at (6.29032258064516,3) {Python};
\node [lang] (Ruby) at (15,0) {Ruby};
\draw [->,dotted,thick,colormedium,bend right=20](C-sharp) edge (C);
\draw [->,,colormedium](C) edge (Go);
\draw [->,,colormedium](C) edge (Python);
\draw [->,,colorweak](Haskell) edge (C-sharp);
\draw [->,dotted,thick,colormedium](Python) edge (F-Sharp);
\draw [->,,colormedium,bend right=20](Java) edge (Go);
\draw [->,,colorweak,bend right=20](Go) edge (Ruby);
\draw [->,,colormedium,bend right=20](Haskell) edge (Java);
\draw [->,,colorweak](Java) edge (Python);
\draw [->,,colormedium](Python) edge (Ruby);


==> maxram_exit0_mean_network.tex <==
\node [lang] (C) at (15,3) {C};
\node [lang] (C-sharp) at (-4.61538461538462,0) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (10.3846153846154,0) {Go};
\node [lang] (Haskell) at (-9.23076923076923,0) {Haskell};
\node [lang] (Java) at (-12.6923076923077,3) {Java};
\node [lang] (Python) at (-9.23076923076923,3) {Python};
\node [lang] (Ruby) at (-11.5384615384615,6) {Ruby};
\draw [->,,colorstrong](C-sharp) edge (C);
\draw [->,,colorweak](Haskell) edge (C);
\draw [->,,colorweak](Python) edge (C);
\draw [->,,colorstrong,bend right=20](F-Sharp) edge (C-sharp);
\draw [->,,colorweak](C-sharp) edge (Go);
\draw [->,,colorweak](Java) edge (C-sharp);
\draw [->,dotted,thick,colorweak](Ruby) edge (C-sharp);
\draw [->,,colorweak,bend right=20](Haskell) edge (Go);
\draw [->,,colorweak](Python) edge (Go);


==> maxram_exit0_mean_normrank_network.tex <==
\node [lang] (C) at (15,3) {C};
\node [lang] (C-sharp) at (6.99885624849506,3) {C\#};
\node [lang] (F-Sharp) at (-9.2743197688418,0) {F\#};
\node [lang] (Go) at (13.781904647243,0) {Go};
\node [lang] (Haskell) at (0.60317842523477,0) {Haskell};
\node [lang] (Java) at (-15,0) {Java};
\node [lang] (Python) at (5.94780881290633,0) {Python};
\node [lang] (Ruby) at (-12.2459667710089,3) {Ruby};
\draw [->,,colorstrong](C-sharp) edge (C);
\draw [->,,colorweak](Haskell) edge (C);
\draw [->,,colorweak](Python) edge (C);
\draw [->,,colorstrong](F-Sharp) edge (C-sharp);
\draw [->,,colorweak](C-sharp) edge (Go);
\draw [->,,colorweak](Java) edge (C-sharp);
\draw [->,dotted,thick,colorweak](Ruby) edge (C-sharp);
\draw [->,,colorweak,bend right=20](Haskell) edge (Go);
\draw [->,,colorweak](Python) edge (Go);


==> maxram_exit0_min_network.tex <==
\node [lang] (C) at (15,0) {C};
\node [lang] (C-sharp) at (-0.555555555555555,0) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (9.44444444444445,0) {Go};
\node [lang] (Haskell) at (-12.7777777777778,3) {Haskell};
\node [lang] (Java) at (-10.5555555555556,6) {Java};
\node [lang] (Python) at (-9.44444444444444,0) {Python};
\node [lang] (Ruby) at (-7.22222222222222,3) {Ruby};
\draw [->,,colormedium](Go) edge (C);
\draw [->,,colorstrong,bend right=20](F-Sharp) edge (C-sharp);
\draw [->,,colorweak](C-sharp) edge (Go);
\draw [->,,colorstrong](Java) edge (C-sharp);
\draw [->,,colorweak](Ruby) edge (C-sharp);
\draw [->,dotted,thick,colormedium](F-Sharp) edge (Python);
\draw [->,,colorweak](Haskell) edge (Java);
\draw [->,dotted,thick,colorweak](Haskell) edge (Ruby);
\draw [->,,colormedium](Python) edge (Java);
\draw [->,dotted,thick,colormedium](Python) edge (Ruby);


==> maxram_exit0_min_normrank_network.tex <==
\node [lang] (C) at (15,3) {C};
\node [lang] (C-sharp) at (6.9511308929058,3) {C\#};
\node [lang] (F-Sharp) at (-9.41911163593423,0) {F\#};
\node [lang] (Go) at (13.7846307566536,0) {Go};
\node [lang] (Haskell) at (2.30039058951767,0) {Haskell};
\node [lang] (Java) at (-15,0) {Java};
\node [lang] (Python) at (6.57961667726406,0) {Python};
\node [lang] (Ruby) at (-11.7789990008175,3) {Ruby};
\draw [->,,colormedium](Go) edge (C);
\draw [->,,colorstrong](F-Sharp) edge (C-sharp);
\draw [->,,colorweak](C-sharp) edge (Go);
\draw [->,,colorstrong](Java) edge (C-sharp);
\draw [->,,colorweak](Ruby) edge (C-sharp);
\draw [->,dotted,thick,colormedium,bend right=20](F-Sharp) edge (Python);
\draw [->,,colorweak,bend right=20](Haskell) edge (Go);
\draw [->,,colorweak](Python) edge (Go);
\draw [->,,colorweak](Haskell) edge (Java);
\draw [->,dotted,thick,colorweak](Haskell) edge (Ruby);
\draw [->,,colormedium](Python) edge (Java);
\draw [->,dotted,thick,colormedium](Python) edge (Ruby);


==> maxram_exit0_noFsharp_mean_normrank_network.tex <==
\node [lang] (C) at (15,0) {C};
\node [lang] (C-sharp) at (11.0137393923809,0) {C\#};
\node [lang] (Go) at (11.3357334410933,3) {Go};
\node [lang] (Haskell) at (-15,0) {Haskell};
\node [lang] (Java) at (8.9677087542706,0) {Java};
\node [lang] (Python) at (-0.703133610080451,0) {Python};
\node [lang] (Ruby) at (-3.16189706476617,0) {Ruby};
\draw [->,,colorstrong](C-sharp) edge (C);
\draw [->,,colorweak,bend right=20](Haskell) edge (C);
\draw [->,,colorweak,bend right=20](Python) edge (C);
\draw [->,,colorweak](C-sharp) edge (Go);
\draw [->,,colorweak](Java) edge (C-sharp);
\draw [->,dotted,thick,colorweak,bend right=20](Ruby) edge (C-sharp);
\draw [->,,colorweak](Haskell) edge (Go);
\draw [->,,colorweak](Python) edge (Go);


==> maxram_exit0_noFsharp_min_normrank_network.tex <==
\node [lang] (C) at (14.4677285810038,3) {C};
\node [lang] (C-sharp) at (12.9173402200055,3) {C\#};
\node [lang] (Go) at (15,0) {Go};
\node [lang] (Haskell) at (11.8708354689903,0) {Haskell};
\node [lang] (Java) at (6.08031384299965,0) {Java};
\node [lang] (Python) at (-2.48748176477546,0) {Python};
\node [lang] (Ruby) at (-15,0) {Ruby};
\draw [->,,colorstrong](C-sharp) edge (C);
\draw [->,,colormedium](Go) edge (C);
\draw [->,,colormedium](Haskell) edge (C);
\draw [->,,colorstrong](Java) edge (C-sharp);
\draw [->,,colorweak](Ruby) edge (C-sharp);
\draw [->,,colorweak](Haskell) edge (Java);
\draw [->,dotted,thick,colorweak](Haskell) edge (Ruby);
\draw [->,,colormedium](Python) edge (Java);
\draw [->,dotted,thick,colormedium](Python) edge (Ruby);


==> pfs_exit0_mean_network.tex <==
\node [lang] (C) at (15,0) {C};
\node [lang] (C-sharp) at (15,3) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (13.4210526315789,6) {Go};
\node [lang] (Haskell) at (-11.8421052631579,3) {Haskell};
\node [lang] (Java) at (13.4210526315789,9) {Java};
\node [lang] (Python) at (13.4210526315789,12) {Python};
\node [lang] (Ruby) at (13.4210526315789,15) {Ruby};
\draw [->,,colorweak](F-Sharp) edge (C);
\draw [->,,colormedium](Haskell) edge (C);
\draw [->,,colorweak](F-Sharp) edge (C-sharp);
\draw [->,,colorweak](Haskell) edge (C-sharp);
\draw [->,,colorweak](F-Sharp) edge (Go);
\draw [->,,colorweak](F-Sharp) edge (Java);
\draw [->,,colorweak](F-Sharp) edge (Python);
\draw [->,,colorweak](F-Sharp) edge (Ruby);
\draw [->,,colormedium](Haskell) edge (Go);
\draw [->,,colormedium](Haskell) edge (Java);
\draw [->,,colormedium](Haskell) edge (Python);
\draw [->,,colormedium](Haskell) edge (Ruby);


==> pfs_exit0_min_network.tex <==
\node [lang] (C) at (15,0) {C};
\node [lang] (C-sharp) at (15,3) {C\#};
\node [lang] (F-Sharp) at (0.882352941176471,0) {F\#};
\node [lang] (Go) at (14.4117647058824,6) {Go};
\node [lang] (Haskell) at (-15,0) {Haskell};
\node [lang] (Java) at (14.4117647058824,9) {Java};
\node [lang] (Python) at (13.8235294117647,12) {Python};
\node [lang] (Ruby) at (14.4117647058824,15) {Ruby};
\draw [->,,colorweak](F-Sharp) edge (C);
\draw [->,,colorstrong,bend right=20](Haskell) edge (C);
\draw [->,,colorweak](F-Sharp) edge (C-sharp);
\draw [->,,colorstrong](Haskell) edge (C-sharp);
\draw [->,,colorweak](F-Sharp) edge (Go);
\draw [->,,colorweak](F-Sharp) edge (Java);
\draw [->,,colorweak](F-Sharp) edge (Python);
\draw [->,,colorweak](F-Sharp) edge (Ruby);
\draw [->,,colorstrong](Haskell) edge (Go);
\draw [->,,colorstrong](Haskell) edge (Java);
\draw [->,,colorstrong](Haskell) edge (Python);
\draw [->,,colorstrong](Haskell) edge (Ruby);


==> run_stats_stat_network.tex <==
\node [lang] (C) at (-15,0) {C};
\node [lang] (C-sharp) at (-15,3) {C\#};
\node [lang] (F-Sharp) at (-13.125,6) {F\#};
\node [lang] (Go) at (15,0) {Go};
\node [lang] (Haskell) at (-3.75,0) {Haskell};
\node [lang] (Java) at (-15,9) {Java};
\node [lang] (Python) at (-15,12) {Python};
\node [lang] (Ruby) at (-13.125,15) {Ruby};
\draw [->,dotted,thick,colormedium](C) edge (Haskell);
\draw [->,,colormedium](C-sharp) edge (Haskell);
\draw [->,,colormedium](F-Sharp) edge (Go);
\draw [->,,colormedium](Haskell) edge (Go);
\draw [->,,colorweak](Ruby) edge (Go);
\draw [->,,colormedium](Java) edge (Haskell);
\draw [->,,colormedium](Python) edge (Haskell);


==> scalability_exit0_mean_normrank_network.tex <==
\node [lang] (C) at (15,3) {C};
\node [lang] (C-sharp) at (-13.6903667088171,3) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (14.7318657316933,0) {Go};
\node [lang] (Haskell) at (12.7964900180097,6) {Haskell};
\node [lang] (Java) at (12.991148407863,9) {Java};
\node [lang] (Python) at (9.20019542476147,3) {Python};
\node [lang] (Ruby) at (8.31168333524926,0) {Ruby};
\draw [->,,colorweak](Go) edge (C);
\draw [->,,colorweak](Python) edge (C-sharp);
\draw [->,,colorweak](Ruby) edge (C-sharp);
\draw [->,dotted,thick,colorweak,bend right=20](F-Sharp) edge (Go);
\draw [->,,colorweak](Haskell) edge (Go);
\draw [->,dotted,thick,colorweak](Java) edge (Go);
\draw [->,,colorstrong](Python) edge (Go);
\draw [->,,colorstrong](Ruby) edge (Go);
\draw [->,dotted,thick,colorweak](Haskell) edge (Java);
\draw [->,dotted,thick,colormedium](Python) edge (Java);
\draw [->,dotted,thick,colormedium](Ruby) edge (Java);


==> scalability_exit0_min_network.tex <==
\node [lang] (C) at (15,0) {C};
\node [lang] (C-sharp) at (-4.61538461538462,0) {C\#};
\node [lang] (F-Sharp) at (-9.23076923076923,9) {F\#};
\node [lang] (Go) at (10.3846153846154,0) {Go};
\node [lang] (Haskell) at (-11.5384615384615,6) {Haskell};
\node [lang] (Java) at (-8.07692307692308,12) {Java};
\node [lang] (Python) at (-13.8461538461538,3) {Python};
\node [lang] (Ruby) at (-15,0) {Ruby};
\draw [->,,colorweak](Go) edge (C);
\draw [->,dotted,thick,colorweak](C-sharp) edge (Go);
\draw [->,dotted,thick,colorweak](Python) edge (C-sharp);
\draw [->,,colorweak](Ruby) edge (C-sharp);
\draw [->,dotted,thick,colorweak](F-Sharp) edge (Go);
\draw [->,,colorstrong](Haskell) edge (Go);
\draw [->,dotted,thick,colorweak](Java) edge (Go);
\draw [->,,colorstrong](Python) edge (Go);
\draw [->,,colorstrong,bend right=20](Ruby) edge (Go);
\draw [->,dotted,thick,colormedium](Ruby) edge (Java);


==> scalability_exit0_min_normrank_network.tex <==
\node [lang] (C) at (15,6) {C};
\node [lang] (C-sharp) at (-13.6903667088171,3) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (14.8751772234356,3) {Go};
\node [lang] (Haskell) at (13.0651032685749,0) {Haskell};
\node [lang] (Java) at (12.9925853546385,6) {Java};
\node [lang] (Python) at (9.58855423995096,3) {Python};
\node [lang] (Ruby) at (8.82927156378128,0) {Ruby};
\draw [->,,colorweak](Go) edge (C);
\draw [->,dotted,thick,colorweak](Python) edge (C-sharp);
\draw [->,,colorweak](Ruby) edge (C-sharp);
\draw [->,dotted,thick,colorweak](F-Sharp) edge (Go);
\draw [->,,colorstrong](Haskell) edge (Go);
\draw [->,dotted,thick,colorweak](Java) edge (Go);
\draw [->,,colorstrong](Python) edge (Go);
\draw [->,,colorstrong](Ruby) edge (Go);
\draw [->,dotted,thick,colormedium](Ruby) edge (Java);


==> scalability_exit0_noFsharp_mean_normrank_network.tex <==
\node [lang] (C) at (15,3) {C};
\node [lang] (C-sharp) at (-15,0) {C\#};
\node [lang] (Go) at (14.4484916638146,0) {Go};
\node [lang] (Haskell) at (8.48310761257517,0) {Haskell};
\node [lang] (Java) at (12.0482150714879,3) {Java};
\node [lang] (Python) at (4.18817358263894,3) {Python};
\node [lang] (Ruby) at (1.53246816743614,0) {Ruby};
\draw [->,,colorweak](Go) edge (C);
\draw [->,,colorweak](Python) edge (C-sharp);
\draw [->,,colorweak](Ruby) edge (C-sharp);
\draw [->,,colorweak](Haskell) edge (Go);
\draw [->,dotted,thick,colorweak](Java) edge (Go);
\draw [->,,colorstrong](Python) edge (Go);
\draw [->,,colorstrong,bend right=20](Ruby) edge (Go);
\draw [->,dotted,thick,colorweak](Haskell) edge (Java);
\draw [->,dotted,thick,colormedium](Python) edge (Java);
\draw [->,dotted,thick,colormedium](Ruby) edge (Java);


==> scalability_exit0_noFsharp_min_normrank_network.tex <==
\node [lang] (C) at (15,3) {C};
\node [lang] (C-sharp) at (-15,0) {C\#};
\node [lang] (Go) at (14.7984854859066,0) {Go};
\node [lang] (Haskell) at (9.05132519983172,0) {Haskell};
\node [lang] (Java) at (12.4619267984855,3) {Java};
\node [lang] (Python) at (5.32519983172066,3) {Python};
\node [lang] (Ruby) at (2.08960875052587,0) {Ruby};
\draw [->,,colorweak](Go) edge (C);
\draw [->,dotted,thick,colorweak](Python) edge (C-sharp);
\draw [->,,colorweak](Ruby) edge (C-sharp);
\draw [->,,colorstrong](Haskell) edge (Go);
\draw [->,dotted,thick,colorweak](Java) edge (Go);
\draw [->,,colorstrong](Python) edge (Go);
\draw [->,,colorstrong,bend right=20](Ruby) edge (Go);
\draw [->,dotted,thick,colormedium](Ruby) edge (Java);


==> solutions_count_length.na.zero_network.tex <==
\node [lang] (C) at (2.14285714285714,0) {C};
\node [lang] (C-sharp) at (-10.7142857142857,0) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (2.14285714285714,3) {Go};
\node [lang] (Haskell) at (2.14285714285714,6) {Haskell};
\node [lang] (Java) at (-3.21428571428572,0) {Java};
\node [lang] (Python) at (15,0) {Python};
\node [lang] (Ruby) at (7.5,0) {Ruby};
\draw [->,,colormedium](Java) edge (C);
\draw [->,dotted,thick,colormedium](C) edge (Ruby);
\draw [->,,colormedium](F-Sharp) edge (C-sharp);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colormedium](Java) edge (Go);
\draw [->,,colormedium](Go) edge (Ruby);
\draw [->,,colormedium](Java) edge (Haskell);
\draw [->,,colormedium](Haskell) edge (Ruby);
\draw [->,,colormedium](Ruby) edge (Python);


==> solutions_count_length.na.zero_normrank_network.tex <==
\node [lang] (C) at (0.534950071326671,0) {C};
\node [lang] (C-sharp) at (-9.2225392296719,0) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (-1.00570613409415,0) {Go};
\node [lang] (Haskell) at (0.278174037089867,3) {Haskell};
\node [lang] (Java) at (-3.95863052781741,0) {Java};
\node [lang] (Python) at (15,0) {Python};
\node [lang] (Ruby) at (3.9586305278174,0) {Ruby};
\draw [->,,colormedium,bend right=20](Java) edge (C);
\draw [->,dotted,thick,colormedium](C) edge (Ruby);
\draw [->,,colormedium](F-Sharp) edge (C-sharp);
\draw [->,,colormedium](C-sharp) edge (Java);
\draw [->,,colormedium](Java) edge (Go);
\draw [->,,colormedium,bend right=20](Go) edge (Ruby);
\draw [->,,colormedium](Java) edge (Haskell);
\draw [->,,colormedium](Haskell) edge (Ruby);
\draw [->,,colormedium](Ruby) edge (Python);


==> timeout_binary.timeout.selector_network.tex <==
\node [lang] (C) at (15,0) {C};
\node [lang] (C-sharp) at (-5,0) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (5,0) {Go};
\node [lang] (Haskell) at (0,0) {Haskell};
\node [lang] (Java) at (0,6) {Java};
\node [lang] (Python) at (-5,3) {Python};
\node [lang] (Ruby) at (5,3) {Ruby};
\draw [->,dotted,thick,colorweak,bend right=20](C-sharp) edge (C);
\draw [->,dotted,thick,colorweak,bend right=20](F-Sharp) edge (C);
\draw [->,dotted,thick,colorweak](Python) edge (C);
\draw [->,dotted,thick,colorweak,bend right=20](F-Sharp) edge (Go);
\draw [->,dotted,thick,colorweak](F-Sharp) edge (Ruby);


==> timeout_binary.timeout.selector_normrank_network.tex <==
\node [lang] (C) at (9,12) {C};
\node [lang] (C-sharp) at (3,0) {C\#};
\node [lang] (F-Sharp) at (-15,0) {F\#};
\node [lang] (Go) at (9,0) {Go};
\node [lang] (Haskell) at (15,0) {Haskell};
\node [lang] (Java) at (3,12) {Java};
\node [lang] (Python) at (3,6) {Python};
\node [lang] (Ruby) at (9,6) {Ruby};
\draw [->,dotted,thick,colorweak](C-sharp) edge (C);
\draw [->,dotted,thick,colorweak](F-Sharp) edge (C);
\draw [->,dotted,thick,colorweak](Python) edge (C);
\draw [->,dotted,thick,colorweak,bend right=20](F-Sharp) edge (Go);
\draw [->,dotted,thick,colorweak](F-Sharp) edge (Ruby);

